Conversational Question Answering on Heterogeneous Sources

Conversational question answering (ConvQA) tackles sequential information needs where contexts in follow-up questions are left implicit. Current ConvQA systems operate over homogeneous sources of information: either a knowledge base (KB), or a text corpus, or a collection of tables. This paper addresses the novel issue of jointly tapping into all of these together, this way boosting answer coverage and confidence. We present CONVINSE, an end-to-end pipeline for ConvQA over heterogeneous sources, operating in three stages: i) learning an explicit structured representation of an incoming question and its conversational context, ii) harnessing this frame-like representation to uniformly capture relevant evidences from KB, text, and tables, and iii) running a fusion-in-decoder model to generate the answer. We construct and release the first benchmark, ConvMix, for ConvQA over heterogeneous sources, comprising 3000 real-user conversations with 16000 questions, along with entity annotations, completed question utterances, and question paraphrases. Experiments demonstrate the viability and advantages of our method, compared to state-of-the-art baselines.

==> sections/references.tex <==

General
- Stanford NLP tools
- Stanford NER (stanza)
- NLTK library
- LSH methods
- Wiki2vec paper
- Yago2 KG
- Lucene
- ElasticSearch

KG-encodings
- KOGNAC paper?
- HDT paper
- Adaptive Low-level Storage of Very Large Knowledge Graphs
- C.Weiss et al. Hexastore: Sextuple Indexing for Semantic Web Data Management. PVLDB, 1(1), 2008.
- Don’t Like RDF Reification? Making Statements about Statements Using Singleton Property WWW 2014

Top-k query processing
- Examining the Additivity of Top-k Query Processing Innovations. CIKM 2020: 1085-1094
-> https://dl.acm.org/doi/pdf/10.1145/3340531.3412000
-> recent, includes many references

- Pruned query evaluation using pre-computed impacts. SIGIR 2006: 372-379
-> Vo Ngoc Anh, Alistair Moffat:
-> key paper to cite, Moffat calls "score-ordered" lists "impact-ordered" - impact on the final ranking

- Vo Ngoc Anh, Alistair Moffat:
-> Pruning strategies for mixed-mode querying. CIKM 2006: 190-197
-> consider as well

- C. Buckley, A. F. Lewit: Optimization of Inverted Vector Searches, SIGIR 1985.
-> classical paper, confusing terminology, but close to Fagin-TA
-> Early threshold algorithm, avoids random accesses (FA does not avoid these)

- A survey of top-k query processing techniques in relational database systems. ACM Comput. Surv. 40(4): 11:1-11:58 (2008)
-> Ihab F. Ilyas, George Beskales, Mohamed A. Soliman:
-> best source on rank joins from a DB perspective, complementary to IR

- EASE: An Effective 3-in-1 Keyword Search Method for Unstructured, Semi-structured and Structured Data

- Top-X paper
- Efficient and self-tuning incremental query expansion for top-k query processing paper

Top-k query processing on KG
- Quark-X: An Efficient Top-K Processing Framework for RDF Quad Stores https://dl.acm.org/doi/pdf/10.1145/2983323.2983727
- CONVEX
- D.Wang et al. Top-k Queries on RDF Graphs. Information Sciences,316,2015.



USING HDT: vakulenko2019message


NED
- AIDA
- TagMe
- S-MART
not explicit ned, e.g. AQQU, MaSP; multi-task setups, QAmp: message passing, text-ray
one-shot, some allow top-k but commercial, some papers that do on own, KEQA->own module
 

Top-k


Benchmarks
- LC QuAD 2.0 paper
- CONVEX paper

QA
- PullNet
- Stagg
- Aqqu
- Quint
- Qamp - Vakulenko et al. 2019
- QAnswer
- Template-based Question Answering over RDF Data

Diefenbach et al 2019, QAnswer => using HDT

TAGME + KG (QA system that ELQ uses)


Look at AQQU CN

Facebook AI paper on unified KG+text qa mentions problems with qualifiers (entities in 2-hop!)
